Constructing Data Graphs for Keyword Search

A data graph is a convenient paradigm for supporting keyword search that takes into account available semantic structure and not just textual relevance. However, the problem of constructing data graphs that facilitate both efficiency and effectiveness of the underlying system has hardly been addressed. A conceptual model for this task is proposed. Principles for constructing good data graphs are explained. Transformations for generating data graphs from RDB and XML are developed. The results obtained from these transformations are analyzed. It is shown that XML is a better starting point for getting a good data graph.

==> rdf.tex <==
\subsection{From RDF to Data Graphs}
We briefly touch upon constructing a data graph from
RDF triples. A \emph{triple} has the form
(\textit{subject},~\textit{property},~\textit{object}).\footnote{The
  notion of an object in RDF should not be confused with objects of
  the OCP model.}  Typically, the subject and the object are
\emph{URIs} (uniform resource identifiers), and the object is either a
URI or a \emph{literal} (i.e.,~free text).  RDF is intended to support
uniform terminology of concepts. Therefore, common words are encoded
in a manner that complicates the task of keyword search and consumes
quite a lot of space. For example, the property ``full name'' is
represented by the following:
\url{http://www.w3.org/2000/10/swap/pim/contact#fullName}.
Furthermore, text is fragmented into many triples (e.g.,~there
could be a separate triple for storing each person's title, such as
Dr., Mrs., etc.).  In a naive transformation of RDF data to a
graph, we create a node for each triple and URIs become directed
edges. This approach is likely to yield very thin nodes, causing all
the drawbacks described in Section~\ref{sec:advantages}.  In order to
create an effective data graph for supporting keyword search, we need
to convert cryptic URIs into meaningful text and combine several
triples into a single node. For example, if we have two triples
$(s_1,p_1,o_1)$ and $(s_2,p_2,o_2)$, such that $o_1=s_2$ and $o_2$ is
a literal, then we may represent the information of $(s_2,p_2,o_2)$ as
a property in the node for $(s_1,p_1,o_1)$, instead of creating two
nodes for these triples.  We may also try to apply this idea
recursively in order to generate nested properties. In addition, for
all the triples with the same subject, we should create a single node.
We omit further details due to a lack of space.
